A Posteriori Single- and Multi-Goal Error Control and Adaptivity for Partial Differential Equations

This work reviews goal-oriented a posteriori error control, adaptivity and solver control for finite element approximations to boundary and initial-boundary value problems for stationary and non-stationary partial differential equations, respectively. In particular, coupled field problems with different physics may require simultaneously the accurate evaluation of several quantities of interest, which is achieved with multi-goal oriented error control. Sensitivity measures are obtained by solving an adjoint problem. Error localization is achieved with the help of a partition-of-unity. We also review and extend theoretical results for efficiency and reliability by employing a saturation assumption. The resulting adaptive algorithms allow to balance discretization and non-linear iteration errors, and are demonstrated for four applications: Poisson's problem, non-linear elliptic boundary value problems, stationary incompressible Navier-Stokes equations, and regularized parabolic $p$-Laplace initial-boundary value problems. Therein, different finite element discretizations in two different software libraries are utilized, which are partially accompanied with open-source implementations on GitHub.

==> Figures/ErrorEx1Estimator2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,704){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%
      \put(990,1229){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%
      \put(990,1754){\makebox(0,0)[r]{\strut{}0.0001}}%
      \csname LTb\endcsname%
      \put(990,2279){\makebox(0,0)[r]{\strut{}0.001}}%
      \csname LTb\endcsname%
      \put(990,2804){\makebox(0,0)[r]{\strut{}0.01}}%
      \csname LTb\endcsname%
      \put(990,3329){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%
      \put(990,3854){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%
      \put(990,4379){\makebox(0,0)[r]{\strut{}10}}%
      \csname LTb\endcsname%
      \put(1122,484){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%
      \put(2258,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%
      \put(3394,484){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%
      \put(4531,484){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%
      \put(5667,484){\makebox(0,0){\strut{}100000}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}1e+06}}%
      \put(3962,154){\makebox(0,0){\strut{}\text{DOFs}}}%
      \put(3962,4709){\makebox(0,0){\strut{}Example 1: Errors in $J_c$ and error estimator}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2970,1317){\makebox(0,0)[r]{\strut{} \footnotesize $J_c$}}%
      \csname LTb\endcsname%
      \put(2970,1097){\makebox(0,0)[r]{\strut{} \footnotesize $\eta_h$}}%
      \csname LTb\endcsname%
      \put(2970,877){\makebox(0,0)[r]{\strut{} \footnotesize $O(\text{DoFs}^{-1})$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figures/ErrorEx1Estimator}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nonstandard.tex <==
\subsection{Motivation and Examples of Non-Consistencies}
The basic error identity sketched in
Section~\ref{SubSec:Error-Identity} poses very little assumptions on
the underlying problem and in particular on $u,\tilde u\in U$ and the
adjoints $z,\tilde z\in V$. It can directly be applied to any
$U$-conforming discretization, i.e. $u_h\in U_h\subset U$ and $z_h\in
V_h\subset V$ yielding the identity
%
\begin{equation}\label{ns:id}
  J(u)-J(u_h) = \frac{1}{2}\big(\rho(u_h)(z-z_h) +
  \rho^*(u_h,z_h)(u-u_h)\big) - \rho(u_h)(z_h) + \mathcal{R}^{(3)}.
\end{equation}
%
If we further consider consistent discretizations, i.e. discrete
solutions satisfying
%
\begin{equation}\label{ns:cons}
  \begin{aligned}
    \mathcal{A}(u_h)(\phi_h) &= 0\quad \forall \phi_h\in V_h,\\
    \mathcal{A}'(u_h)(\psi_h,z_h) &= J'(u_h)(\psi_h)\quad \forall \psi_h\in U_h,
  \end{aligned}
\end{equation}
%
and assume for now that the discrete solution $u_h\in U_h$ is indeed a
solution and no iteration error remains,~\eqref{ns:id} simplifies to
%
\begin{equation}\label{ns:id1}
  J(u)-J(u_h) = \frac{1}{2}\big(\rho(u_h)(z-z_h) +
  \rho^*(u_h,z_h)(u-u_h)\big) + \mathcal{R}^{(3)}.
\end{equation}
%
This gives rise to the classical formulation of the adjoint error
identity~\cite{BeRa01} that, using Galerkin orthogonality, allows to
localize the error by replacing the approximation errors $u-u_h$ and
$z-z_h$ by any interpolation $I_h u\in U_h$ and $I_h z\in V_h$
%
\begin{equation}\label{ns:id2}
  J(u)-J(u_h) = \frac{1}{2}\big(\rho(u_h)(z-I_h z) +
  \rho^*(u_h,z_h)(u-I_h u)\big) + \mathcal{R}^{(3)}.
\end{equation}
%
% TW, Mar 30: bis hierhin gut.
Besides conformity and consistency of the discretization, the
fundamental assumption is the variational principle defining the
solution $u\in U$ and its adjoint $z\in V$.

In the following paragraphs, we examine various problems in which one
or more of these assumptions are violated. One straightforward example is
the realization of Dirichlet conditions. Assume that the proper
solution space would be
\[
u\in U = u^D+H^1_0(\Omega),
\]
where $u^D\in H^1(\Omega)$ is the extension of some boundary data
$g\in H^\frac{1}{2}(\partial\Omega)$. The discrete finite element
realization would find
\[
u_h\in U_h = I_h u^D + U_h^0,
\]
where $U_h^0\subset H^1_0(\Omega)$ has homogeneous Dirichlet data, but
where $I_h u^D\neq u^D$ such that $U_h\not\subset U$. An
even simpler example is the weak  enforcement of boundary conditions
by Nitsche's method~\cite{Ni71}, where, in general, $u_h\neq 0$ on the
discrete boundary and hence $u_h\not\in H^1_0(\Omega)$. Further
examples leading to non-conforming discretizations are approximations
on curved domains, where $\Omega\neq \Omega_h$~\cite{MinakowskiRichter2019}, non-conforming finite
elements such as the Crouzeix-Raviart element \cite{CrouRa73} or discontinuous
Galerkin methods \cite{Ri08,DiErn2012} for elliptic problems.

Another potential source of problems lies in the non-consistency of
the discrete formulation. While consistency is required to use
Galerkin orthogonality for localization in the spirit
of~\eqref{ns:id2}, it is not essential for the path outlined in
Section~\ref{Sec:single-goal} as the error identity contains the term
$\rho(\tilde u)(\tilde z)$, which, on the one hand, stands for
iteration errors, but which also includes all non-conformity
errors. Classical sources of non-consistency are stabilized finite
element methods, where the discrete variational formulation must be
enriched. Examples are transport stabilizations such as streamline diffusion for
a simple diffusion transport problem
%
\begin{equation}\label{ns:stab}
  \mathcal{A}_h(\cdot)(\cdot) = \mathcal{A}(\cdot)(\cdot)+\mathcal{S}(\cdot)(\cdot),
\end{equation}
%
where
%
\begin{equation}\label{ns:stab:sd}
  \mathcal{A}_h(u)(\phi) = \underbrace{(\nabla u,\nabla \phi) + (\beta\cdot\nabla
    u,\phi)}_{={\mathcal A}(u)(\phi)} +
  \underbrace{(\delta_h\beta\cdot\nabla u,\beta\cdot\nabla
    \phi)}_{={\mathcal S}(u)(\phi)}
\end{equation}
%
and where the solution $u\in U$ to $\mathcal{A}(u)(\phi)=0$ for all
$\phi\in V$ does not satisfy the discrete problem
$\mathcal{A}_h(u)(\phi)=0$. Other examples are stabilizations of
saddle-point problems such as local
projections~\cite{BeckerBraack2001}. Non-consistency is also relevant
for time-dependent problems. While the DWR
estimator can directly be applied to space-time Galerkin methods as
discussed in Section~\ref{Sec:single-goal}, Galerkin time
discretizations might not be favorable in terms of computational
complexity. Instead, efficient time-stepping methods are used for
simulation and their similarity to certain Galerkin space-time
discretization is utilized for error estimation 
only~\cite{MeiRi14,MeidnerRichter2015}.
 

The idea of different methods in simulation and theoretical error
analysis can be taken even further. For example, the error estimator
can in principle be applied to discrete solutions that are not based
on variational principles at all, but are obtained using finite
volume methods~\cite{CHEN201469} or neural networks~\cite{minakowski2021error}. 

% TW, Mar 30: bis hierhin gut.

\subsection{Estimating the Consistency Error}
\label{SubSec:consistency}

As before, let $\mathcal{A}(\cdot)(\cdot)$ be the variational semi-linear form
describing the problem at hand. Then, we have: Find 
% AS: fehlt bei den VF hier ein Find ?
% TW, Mar 31: done. (BE's Vorschlag noch erweitert.)
{%
\begin{equation}
u\in U: \quad \mathcal{A}(u)(v) = 0\quad \forall v\in V.
\end{equation}
}%
Then, $u_h\in U_h\subset U$ shall be the discrete approximation that
is given in the modified variational form 
\begin{equation}
u_h\in U_h\subset U\quad \mathcal{A}_h(u_h)(v_h) = 0\quad \forall v_h\in V_h,
\end{equation}
where we assume that consistency does not hold, i.e. in the general case we have
\begin{equation}
\mathcal{A}_h(u)(v_h) \neq 0\quad\forall v_h\in V_h.
\end{equation}
%
For the following we assume that the discrete variational form can be written as
$\mathcal{A}_h(\cdot)(\cdot)=\mathcal{A}(\cdot)(\cdot)+\mathcal{S}_h(\cdot)(\cdot)$, and that the discrete adjoint problem is given by:
%
\begin{equation}
  \text{Find  $z_h\in V_h$:} \quad \mathcal{A}_h'(u_h)(v_h,z_h) = J'(u_h)(v_h)\quad\forall v_h\in U_h,
\end{equation}
%
with $\mathcal{A}_h'(\cdot)(\cdot,\cdot) = \mathcal{A}'(\cdot)(\cdot,\cdot) +
\mathcal{S}^*_h(\cdot)(\cdot,\cdot)$, where $\mathcal{S}^*_h$ is not necessarily the derivative of $\mathcal{S}_h(\cdot,\cdot)$. 

\begin{Theorem}\label{thm: Error Representation Consistency}
  Let $u\in U$ and $z\in V$ be primal and adjoint solutions such that
  \[
  \mathcal{A}(u)(v) = 0\quad\forall v\in V,\quad
  \mathcal{A}'(u)(v,z) = J'(u)(v)\quad\forall v\in U.
  \]
  Further, let  $u_h\in U_h\subset U$ and $z_h\in  V_h\subset V$ be primal and adjoint discrete approximations such that
  \[
  \mathcal{A}_h(u_h)(v_h) \approx 0\quad\forall v_h\in V_h,\quad
  \mathcal{A}_h'(u_h)(v_h,z_h) \approx J'(u_h)(v_h)\quad\forall v_h\in U_h,
  \]
  where
  \begin{equation}\label{ns:stabform}
    \mathcal{A}_h(u)(v) = \mathcal{A}(u)(v) + \mathcal{S}_h(u)(v),\quad
    \mathcal{A}'_h(u)(v,z) = \mathcal{A}'(u)(v,z) + \mathcal{S}_h^*(u)(v,z).
  \end{equation}
  %
  Then, the following error representation holds
  \begin{equation} \label{eq:ConsistencyError}
    J(u)-J(u_h)= \frac{1}{2}\left(\rho(u_h)(z-z_h)+\rho^*(u_h,z_h)(u-u_h)\right) - \rho_h(u_h)(z_h)-\mathcal{S}_h(u_h)(z_h) + \mathcal{R}^{(3)}.
  \end{equation}
  Here, $\rho(\cdot)(\cdot),\rho^*(\cdot,\cdot)(\cdot)$ and $\mathcal{R}^{(3)}$ are defined as in Theorem~\ref{thm: error identity}, whereas
  \[
  \rho_h(u)(v) = -A_h(u)(v),\quad \rho_h^*(u,z)(v) = J'(u)(v)-A'(u)(v,z).
  \]
  Given interpolations $I_h:U\to U_h$ and $I_h^*:V\to V_h$, the localization of this error identity reads
  \begin{multline} \label{eq:ConsistencyErrorLocal}
    J(u)-J(u_h)= \frac{1}{2}\left(\rho(u_h)(z-I_h^*z)+\rho^*(u_h,z_h)(u-I_hu) \right)\\
    -\rho_h(u_h)(z_h) 
    +\frac{1}{2}\left(\rho_h(u_h)(I_h^*z - z_h)+\rho_h^*(u_h,z_h)(I_h^*u - u_h)\right)\\
    -\frac{1}{2}\left(\mathcal{S}_h(u_h)(I_h^*z - z_h)+\mathcal{S}_h^*(u_h)(I_h^*u - u_h,z_h)\right) - \mathcal{S}_h(u_h)(z_h)
    + \mathcal{R}^{(3)}.
  \end{multline}
  \begin{proof}
    The error identity~\eqref{eq:Error Representation} of Theorem~\ref{thm: error identity} does not require consistency and is directly applicable
    \[
    J(u)-J(u_h)= \frac{1}{2}\left(\rho(u_h)(z-z_h)+\rho^*(u_h,z_h)(u-u_h)\right) - \rho(u_h)(z_h) + \mathcal{R}^{(3)}.
    \]
  Using~\eqref{ns:stabform},~\eqref{eq:ConsistencyError} directly follows. 
  %

  If we want to exploit Galerkin orthogonality to localize by means of replacing the approximation errors $u-u_h$ and $z-z_h$ by interpolation weights, we introduce $\pm \rho(u_h)(z_h-I_h^*z)$ and $\pm \rho^*(u_h)(u_h-I_h u,z_h)$, and we obtain
  %
  \begin{multline}\label{ns:7}
    J(u)-J(u_h)= \frac{1}{2}\left(\rho(u_h)(z-I_h^*z)+\rho^*(u_h,z_h)(u-I_hu) \right)
    -\rho_h(u_h)(z_h)  - \mathcal{S}_h(u_h)(z_h)\\
    +\frac{1}{2}\left(\rho(u_h)(I_h^*z - z_h)+\rho^*(u_h,z_h)(I_h^*u - u_h)\right)
    + \mathcal{R}^{(3)}.
  \end{multline}
  %
  We further use~\eqref{ns:stabform} to split $\rho(\cdot)(\cdot) = \rho_h(\cdot)(\cdot)-\mathcal{S}_h(\cdot)(\cdot)$, and likewise $\rho^*(\cdot,\cdot)(\cdot)$ to separate the error identity into weighted residuals, iteration errors and consistency errors to reach~\eqref{eq:ConsistencyErrorLocal}.
  \end{proof}
\end{Theorem}
% TW, Mar 30: bis hierhin. Das ist ein schoenes Resultat. 


The error identities~\eqref{eq:ConsistencyError} and~\eqref{eq:ConsistencyErrorLocal} now consist of five parts: primal and dual weighted residuals, the discrete iteration error, the non-consistency error and, finally, the remainder. Apart from the remainder, all other terms can be evaluated numerically, where for the residuals one of the approximations discussed in Section~\ref{SubSec:EEEnriched} or Section~\ref{SubSec:Interpolation} has to be used. The iteration errors vanish if the algebraic problems are solved to sufficient precision.

\begin{Remark}[Consistency remainders]
  The two additional non-consistency terms appearing in~\eqref{ns:7} can not be directly evaluated, as they depend on the unknown exact solutions $u\in U$ and $z\in V$. However, they are usually negligible, as they carry an additional order compared to the consistency term $S_h(u_h)(z_h)$. As an example we consider the streamline diffusion stabilization~\eqref{ns:stab:sd}, where
  \begin{equation}
  \mathcal{S}_h(u_h,v_h) = (\delta_h \beta\cdot\nabla u_h,\beta\cdot\nabla v_h)
  \end{equation}
  and $\mathcal{S}^*_h(u_h)(v_h,z_h) = \mathcal{S}_h(v_h,z_h)$. While $\mathcal{S}_h(u_h)(z_h)$ can simply be estimated as
  \begin{equation} \label{ns:x}
  \big|\mathcal{S}_h(u_h)(z_h)\big| \le c |\delta_h|\,\|\nabla u_h\|\cdot \|\nabla z_h\|,
  \end{equation}
  primal and adjoint    consistency remainders give rise to
  \begin{equation} 
  \big|\mathcal{S}_h(u_h)(I_h^*-z_h)\big| \le c |\delta_h|\,\|\nabla u_h\|\cdot
  \big(\|\nabla (z-z_h)\|+\|\nabla (z-I_h^*z)\|\big),
  \end{equation}
  which is of higher order as compared to the main consistency term~\eqref{ns:x}.
\end{Remark}

% TW, Mar 30: bis hierhin.

\subsubsection{Consistency Error in Galerkin Time-Stepping Methods}

Besides stabilization techniques, another typical application of tracking consistency 
errors in error estimation is found in time-stepping methods. To illustrate this, let $u'(t) = f(t,u(t))$ be a given scalar initial value problem on $I=(0,T)$ with $u(0)=u_0$. By $0=t_0<t_1<\dots<t_N=T$ we introduce discrete points in time, where we uniformly assume $\Delta t=t_n-t_{n-1}$ for simplicity of notation only. Simple time-stepping schemes like the backward Euler method
\begin{equation}\label{ns:ie}
u^n + \Delta t f(t_n,u^n) = u^{n-1}
\end{equation}
find their counterpart in Galerkin time-stepping methods such as introduced by Eriksson,  Estep, Hansbo, and Johnson~\cite{ErikssonEstepHansboJohnson1995} as well as Thom{\'e}e~\cite{Thomee1997}. Time-stepping methods and Galerkin methods must still be seen as two distinct methods. Introducing the discontinuous space
%
\begin{equation}
  U_h = \{ v\in L^2(I) | \; v(t_0)\in\mathbb{R},\; v\big|_{(t_{n-1},t_n]}\in\mathbb{R},\; n=1,\dots,N\},
\end{equation}
%
the backward Euler method~\eqref{ns:ie} can be formulated as to find $u_h\in U_h$ such that
\begin{equation}
A_h(u_h)(v_h) = 0\quad\forall v_h\in V_h=U_h
\end{equation}
with the fully discrete variational formulation
\begin{equation}\label{var:be}
  A_h(u_h)(v_h) =\left(u_h(t_0)-u_0\right)\cdot v_h(t_0) +  \sum_{n=1}^N \left(u_h(t_n)-u_h(t_{n-1}) + \Delta t f\left(t_n,u(t_n)\right)\right)\cdot v_h(t_n). 
\end{equation}
In contrast, the corresponding discontinuous Galerkin approach also defines $u_h\in U_h$ given by
\begin{equation}
A(u_h)(v_h) = 0\quad\forall v_h\in U_h,
\end{equation}
where the continuous variational form is 
\begin{multline}\label{var:dg}
  A(u_h)(v_h) =\left(u_h(t_0)-u_0\right)\cdot v_h(t_0)\\
  +  \sum_{n=1}^N\left\{ \left(u_h(t_n)-u_h(t_{n-1}\right)\cdot v_h(t_n)
  +\int_{t_{n-1}}^{t_n} f(t,u_h(t))\cdot v_h(t)\right\}.
\end{multline}
Both forms,~\eqref{var:be} and~\eqref{var:dg}, only differ by numerical quadrature. However, as~\eqref{var:be} is based on the box rule which has the same order of convergence as the backward Euler method itself, both discrete approaches must be considered substantially different.

The consistency error can be introduced as $\mathcal{S}_h(u)(z) = A_h(u)(z)-A(u)(z)$ and for the Euler method we obtain
\begin{equation}\label{var:dg_consistency}
  \begin{aligned}
    |S(u_h)(z_h)| &= \sum_{n=1}^N \int_{t_{n-1}}^{t_n} \Delta t\cdot |z_h(t_n)|\cdot \left| f(t_n,u_h(t_n)) - \int_{t_{n-1}}^{t_n} f(t,u_h(t))\,\text{d}t\right|\\
    &= \sum_{n=1}^N \int_{t_{n-1}}^{t_n} \Delta t^2\cdot |z_h(t_n)|\cdot \left| f'(\xi_n) + O(\Delta t)\right|,
  \end{aligned}
\end{equation}
as $u_h(t)=u_h(t_n)$ for $t\in (t_{n-1},t_n]$ and assuming that
$f(\cdot)$ is differentiable. This yields the same order as the
truncation error of the backward Euler method itself. The
consistency term cannot be neglected, but its evaluation must be
included as part of the error identity.
  
If efficient time-stepping methods are used in simulations and a posteriori error estimation based on the DWR method is applied, the consistency error hence has to be tracked. For details and applications to flow problems discretized by the Crank-Nicolson scheme 
and Fractional-Step-$\theta$ method, 
we refer to~\cite{MeiRi14,MeidnerRichter2015,Ri17_fsi}. 

% TW, Mar 30: bis hierhin. Gut (smaller typos corrected.)

\subsection{Estimating the Non-Conformity Error}
\label{SubSec:conformity}

The application to non-conforming discretizations is more cumbersome and there is no one standard approach. This is already due to the fact that even the definition of the error $u-u_h$ can be difficult. This is the case, for example, if $u$ is given on a domain $\Omega$ and $u_h$ on a discretized domain $\Omega_h$. In this case, one remedy could be to limit all considerations to the intersection $\Omega\cap\Omega_h$, see for instance~\cite{MinakowskiRichter2019}.

Since the sources of non-conformity are manifold, we discuss two examples in the following, first classical non-conforming finite element approaches and then discretizations that are not based on variational principles at all.

\subsubsection{Non-Conforming Finite Elements}

Let $u\in U$ be the solution to
%
\begin{equation}
  \mathcal{A}(u)(v) = 0\quad\forall v\in V.
\end{equation}
%
By $U_h\not\subset U$ and $V_h\not\subset V$ we denote a
non-conforming finite element discretization. As specific problem, 
%we might have 
consider a $H^1$-elliptic problem in mind with $U=V=H^1_0(\Omega)$
and where $U_h=V_h$ is the non-conforming Crouzeix-Raviart element. We
must assume that the variational form $\mathcal{A}(\cdot)(\cdot)$ is
also defined in $U_h\times U_h$ and elliptic. Hence, we introduce
$X=U\cup U_h$ and consider $\mathcal{A}:X\times X\to\mathbb{R}$ and,
likewise, we assume that the functional is defined on
$J:X\to\mathbb{R}$, which is a limitation as, for instance, line
integrals along mesh edges are not well defined on $U_h$.

The direct application of Theorem~\ref{thm: error identity} is not possible, since the fact that the residual of the continuous solution disappears in a conformal discretization was exploited here, namely $\mathcal{L}'(u,z)(u-u_h,z-z_h)=0$. 
This is not necessarily the case for a non-conforming discretization. Instead, what remains is the term
\begin{equation}
  \mathcal{L}'(u,z)(u-u_h,z-z_h)=
  \frac{1}{2}\left(
  -\mathcal{A}(u)(z-z_h) + J'(u)(u-u_h) - \mathcal{A}'(u)(u-u_h,z)\right). 
\end{equation}
Its meaning must be considered on a case-by-case basis. For
%the Laplace equation 
Poisson's problem $\mathcal{A}(u)(v) = (\nabla u,\nabla v)-(f,v)$, the error identity from Theorem~\ref{thm: error identity} reads as
\begin{multline}
  J(u-u_h) = \frac{1}{2}\left(\rho(u_h)(u-u_h)+\rho^*(u_h,z_h)(z-z_h)\right) - \rho(u_h)(z_h)\\
  \frac{1}{2}\left(
  (f,z-z_h) - \left(\nabla u,\nabla (z-z_h)\right)+ J'(u)(u-u_h) - \left(\nabla (u-u_h),\nabla z\right)\right)
  +\mathcal{R}^{(3)}. 
\end{multline}
%
Using integration by parts, these terms get
\begin{equation}
  \begin{aligned}
    (f,z-z_h) - \left(\nabla u,\nabla (z-z_h)\right) &= \sum_{{K\in \mathcal{T}_h}} \langle \partial_n u,[z_h]\rangle_{{\partial K}}\\
    J'(u)(u-u_h) - \left(\nabla (u-u_h),\nabla z\right)&= \sum_{{K\in \mathcal{T}_h}} \langle \partial_n z,[u_h]\rangle_{{\partial K}},
  \end{aligned}
\end{equation}
%
where $[\cdot]$ denotes the jump over the element's edge $\partial K$ 
and $\mathcal{T}_h$ is the decomposition of $\Omega_h$. 
%Bernhard: Bitte gegenlesen ob das richtig ist.
This term exactly measures the non-conformity of the discrete approximations $u_h$ and $z_h$. 
Instead of a rigorous bound, it can be estimated based on replacing $\partial_n u$ and $\partial_n z$ by discrete reconstructions, see~\cite{Grajewski} for a similar procedure. 
We refer to~\cite{MaVohYou20} for a detailed presentation of a goal-oriented error estimator for different conforming and non-conforming discretizations.

% TW, Mar 30: bis hierhin. Smaller typos corrected. One question `must be'?!

\subsubsection{Non-Variational Discretization Methods}

Finally, we explore 
% the extend
to which extend the error estimator can be
applied to discretizations that cannot be written in the form of a
variational formulation at all. These could be, for example, finite
difference methods, or the approximation of differential equations
with neural networks like \emph{Physics Informed Neural Networks
(PINNs)} such as the \emph{Deep Ritz} method~\cite{EYu2017}. In both cases, the discrete approximation $u_h$ cannot be represented by a variational formulation.
Once again, we cannot rely on a uniform theoretical principle, but must argue on a case-by-case basis.

What we require in any case is the embedding of the discrete solution
$u_h$ into a function space $\mathcal{E}:u_h\mapsto U_h$ that is in some sense compatible, meaning that it is either conforming $U_h\subset U$ or that the variational form 
can be extended onto $X:=U\cup U_h$ such as in the case of the non-conforming Crouzeix-Raviart element. Considering finite difference approximations $\mathcal{E}(u_h) = I_h u_h$, the interpolation into a usual finite element space is one conforming option. In this setting, the original error identity from Theorem~\ref{thm: error identity} can directly be applied:
%
\begin{Theorem}[Error identity for conforming embeddings]
Let $u\in U$ and $z\in V$ be the primal and dual solutions. Let $u_h$ and $z_h$ be any discrete approximations. Further, let
\begin{equation}
\mathcal{E}:u_h\mapsto U_h\subset U,\quad
\mathcal{E}^*:z_h\mapsto V_h\subset V,
\end{equation}
be embeddings of the discrete approximations into subspaces. Then, it holds
\begin{multline}
J(u)-J(\mathcal{E}(u_h)) = \frac{1}{2}
\left(
\rho\left(\mathcal{E}(u_h)\right)\left(z-\mathcal{E}^*(z_h)\right)+
\rho^*\left(\mathcal{E}(u_h),\mathcal{E}^*(z_h)\right)\left(u-\mathcal{E}(u_h)\right)\right)\\
-\rho\left(\mathcal{E}(u_h)\right)\left(\mathcal{E}^*(z_h)\right) + \mathcal{R}^{(3)}.
\end{multline}
\end{Theorem}
%
Like all previous error identities, this one suffers from the need 
to approximate numerically the primal and adjoint solutions $u\in U$ and $z\in V$. Furthermore, the embeddings $\mathcal{E}(u_h)$ and $\mathcal{E}^*(z_h)$ must be available for numerical evaluation. But most important, the error estimator is still based on variational principles although the discrete approximations $u_h$ and $z_h$ can be obtained in completely different ways. To evaluate the error, integrals over the computational domains containing the embeddings $\mathcal{E}(u_h)$ and $\mathcal{E}^*(z_h)$ must be computed. This will either require a mesh, which is all but trivial, if the choice of discretization method - e.g. smoothed particle hydrodynamics - was motivated as being mesh-free, or, if, for instance, neural networks are chosen for high-dimensional problems. Resorting to simple Monte Carlo quadrature avoids this problem, but it brings along a substantial quadrature error. We refer to~\cite{minakowski2021error} for a first discussion on this mostly open topic.

% TW, Mar 30: gut.

